Fairness, Accuracy, and Unreliable Data

This thesis investigates three areas targeted at improving the reliability of machine learning; fairness in machine learning, strategic classification, and algorithmic robustness. Each of these domains has special properties or structure that can complicate learning. A theme throughout this thesis is thinking about ways in which a `plain' empirical risk minimization algorithm will be misleading or ineffective because of a mis-match between classical learning theory assumptions and specific properties of some data distribution in the wild. Theoretical understanding in eachof these domains can help guide best practices and allow for the design of effective, reliable, and robust systems.

==> mal_ethics.tex <==
In this Section we will conduct the NeurIPS Ethics Review, a critical and important step in helping ensure beneficial research outcomes. 
The research process of this paper did not cause any direct harm to persons, since our work is theoretical and mathematical, so our ethical analysis focuses on \emph{Societal Impact and Potential Harmful Consequences}. 

The areas of concern on the NeurIPS guidelines for social impact are safety, security, discrimination, surveillance, deception and harassment, environmental, humans rights, and bias and fairness.

Of this list, \emph{discrimination, and bias and fairness} are the most relevant to our work. 
We will consider these notions together.

This section of the Ethics Review directs us to consider `known or anticipated consequences of research.'
The high level idea in our paper is studying and improving the robustness of fairness constrained learning in the presence of malicious noise.
Our work is a step towards models that are robust to malicious noise, which would ideally result in fair \emph{and} accurate learning systems. 
This paper also exposes when models are inevitably fragile, and thus directs actors towards a different solution concept or system.
These two threads would ideally have a positive benefit in mitigating discrimination and bias.

However, there exists a certain constant risk that mathematical models of bias (and models learned on data) are mismatched with
the underlying empirical reality and that when deployed supposedly unambiguously beneficial interventions can be harmful.
The malicious noise model is intentionally a worst case model with quite capacious assumptions, so we believe our results are quite general and would not fall in this trap; but these concerns are worth keeping in mind when considering a new deployment.
In particular, the field of fairness constrained learning needs more experimental verification.

Despite these risks, we thoroughly believe that it is critical to study fairness in learning since different demographic groups exist in the real world  and machine learning can affect those groups differently.  
Theoretical work like ours is critical to exposing fundamental trade-offs and 
baselines that can help craft effective fairness interventions.

We are confident our work passes high ethical standards and is a net ethical benefit to society at large. 

==> mal_macros.tex <==
%%%%% Macros :
% All Bracketting commands :
\newcommand{\inbrace}[1]{\left \{ #1 \right \}}
\newcommand{\inparen}[1]{\left ( #1 \right )}
\newcommand{\insquare}[1]{\left [ #1 \right ]}
\newcommand{\inangle}[1]{\left \langle #1 \right \rangle}
\newcommand{\infork}[1]{\left \{ \begin{matrix} #1 \end{matrix} \right .}
\newcommand{\inmat}[1]{\begin{matrix} #1 \end{matrix}}
\newcommand{\inbmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\insqmat}[1]{\insquare{\begin{matrix} #1 \end{matrix}}}
\newcommand{\inabs}[1]{\begin{vmatrix} #1 \end{vmatrix}}
\newcommand{\norm}[2]{\begin{Vmatrix} #2 \end{Vmatrix}_{#1}}
\newcommand{\bra}[1]{\left \langle #1 \right |}
\newcommand{\ket}[1]{\left | #1 \right \rangle}
\newcommand{\braket}[2]{\left \langle #1 \right | \! \left . #2 \right \rangle}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}

\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}

% Floor, Ceiling :
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}

% Math operators :
%\newcommand{\SET}[1]{\inbrace{#1}}
\newcommand{\setdef}[2]{\set{#1 : #2}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\expect}{\mathbb{E}}
%\DeclareMathOperator*{\Ex}{\mathbb{E}}
%\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator*{\Ex}{\mathds{E}}
\DeclareMathOperator*{\E}{\mathds{E}}
\DeclareMathOperator*{\Var}{\mathsf{Var}}
\DeclareMathOperator*{\Cov}{\mathsf{Cov}}
\DeclareMathOperator*{\Stab}{\mathsf{Stab}}
\DeclareMathOperator*{\Prob}{Pr}

\renewcommand{\Pr}{\mathbf{Pr}}

\newcommand{\wtilde}[1]{\widetilde{#1}}
\newcommand{\what}[1]{\widehat{#1}}

\newcommand{\dTV}{d_{\mathrm{TV}}}

\newcommand{\bit}{\set{0,1}}
\newcommand{\sbit}{\set{1, -1}}
\newcommand{\eps}{\varepsilon}

% Letters in Mathrm:
\newcommand{\sAND}{\ \mathrm{and} \ }
\newcommand{\sOR}{\ \mathrm{or} \ }
\newcommand{\sXOR}{\ \mathrm{xor} \ }
\newcommand{\sIF}{\ \mathrm{if} \ }

% Letters in MathBB :
%\newcommand{\bbC}{{\mathbb C}}
%\newcommand{\bbE}{{\mathbb E}}
%\newcommand{\bbF}{{\mathbb F}}
%\newcommand{\bbN}{{\mathbb N}}
%\newcommand{\bbP}{{\mathbb P}}
%\newcommand{\bbQ}{{\mathbb Q}}
%\newcommand{\bbR}{{\mathbb R}}
%\newcommand{\bbS}{{\mathbb S}}
%\newcommand{\bbZ}{{\mathbb Z}}
%\newcommand{\bbA}{{\mathbb A}}
%\newcommand{\bbB}{{\mathbb B}}

% Bold letters :
\let\boldm\bm
%\renewcommand{\bm}{{\boldm m}}
\newcommand{\ba}{{\boldm a}}
\newcommand{\bb}{{\boldm b}}
\newcommand{\bc}{{\boldm c}}
\newcommand{\bd}{{\boldm d}}
\newcommand{\be}{{\boldm e}}
\newcommand{\br}{{\boldm r}}
\newcommand{\bs}{{\boldm s}}
\newcommand{\bt}{{\boldm t}}
\newcommand{\bu}{{\boldm u}}
\newcommand{\bv}{{\boldm v}}
\newcommand{\bw}{{\boldm w}}
\newcommand{\bx}{{\boldm x}}
\newcommand{\by}{{\boldm y}}
\newcommand{\bz}{{\boldm z}}
\newcommand{\tbx}{\Tilde{{\boldm x}}}
\newcommand{\tby}{\Tilde{{\boldm y}}}
\newcommand{\tbz}{\Tilde{{\boldm z}}}

\newcommand{\bA}{{\boldm A}}
\newcommand{\bB}{{\boldm B}}
\newcommand{\bP}{{\boldm P}}
\newcommand{\bM}{{\boldm M}}
\newcommand{\bU}{{\boldm U}}
\newcommand{\bV}{{\boldm V}}
\newcommand{\bW}{{\boldm W}}
\newcommand{\bX}{{\boldm X}}
\newcommand{\bY}{{\boldm Y}}
\newcommand{\bZ}{{\boldm Z}}

\newcommand{\bsigma}{{\boldsymbol \sigma}}
\newcommand{\balpha}{{\boldsymbol \alpha}}
\newcommand{\bbeta} {{\boldsymbol \beta}}

% Letters in Cal :
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\B}{\mathrm{B}}

\newcommand{\sfO}{{\mathsf{O}}}
\newcommand{\ERM}{\textsf{ERM}\xspace}
\newcommand{\RERM}{\textsf{RERM}\xspace}
\newcommand{\VRM}{\textsf{VRM}\xspace}
\newcommand{\IRM}{\textsf{IRM}\xspace}
%\newcommand{\ind}{\mathbbm{1}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\Risk}{{\rm R}}
\newcommand{\err}{{\rm err}}
\newcommand{\vc}{{\rm vc}}
\newcommand{\Tdim}{{\rm Tdim}}
\newcommand{\Ldim}{{\rm lit}}
\newcommand{\MAJ}{{\rm MAJ}}
%\newcommand{\co}{{\rm co}}
\newcommand{\im}{{\rm im}}
\newcommand{\alg}[1]{\textup{\textsf{#1}}\xspace}
\newcommand{\Mre}{m_0}
\newcommand{\OPT}{\mathsf{OPT}}
\newcommand{\OPTDMax}{\mathsf{OPT}^{\mathcal{D}}_{\max}}
\newcommand{\OPTSMax}{\mathsf{OPT}^S_{\max}}
%\newcommand{\OPT}{\mathbb{OPT}}
%\newcommand{\OPTDMax}{\mathbb{OPT}^{\mathcal{D}}_{\max}}
%\newcommand{\OPTSMax}{\mathbb{OPT}^S_{\max}}
\newcommand{\Rob}{{\rm Rob}}
\newcommand{\CAS}{{\rm CAS}}
\newcommand{\wrt}{with respect to }
\renewcommand{\vec}[1]{\mathbf{#1}}
% Model and Algorithm Names
\newcommand{\smodel}{{Perfect Attack Oracle model}\xspace}
\newcommand{\cycalg}{{CycleRobust}\xspace}
\newcommand{\rlua}{{RLUA}\xspace}
\newcommand{\RLoss}{\ell^{\text{rob}}}

\newcommand{\removed}[1]{}
\newcommand{\omarnote}[1]{\todo[color=green,size=\scriptsize]{Omar:: {#1}}}

% Colors
\newcommand{\Maroon}[1]{\textcolor{Maroon}{#1}}

\newcommand{\RoBoost}{\hyperref[alg:cascade]{\textup{$\beta$-RoBoost}}}
\newcommand{\URoBoost}{\hyperref[alg:unlabeled]{\textup{$\beta$-URoBoost}}}

\newcommand{\alphaBoost}{\hyperref[alg:alphaboost]{\textup{$\alpha$-Boost}}}
\DeclareMathOperator{\opt}{OPT}

==> sup-5_seperablecosts.tex <==
\label{subsec:sepCosts}
Previous work \cite{hardt2016strategic} exhibits multiple positive results when the cost function is separable, a more well-behaved notion than when the cost is a metric. 
For reference, 
\begin{definition}
    A cost function $c(x,y)$ is called separable if it can be written as $c(x,y) = \max \{0, c_2(y) - c_1 (x)\}$, for functions $c_1, c_2 : \mathcal{X} \rightarrow \mathbb{R}$ and $c_1( \mathcal{X}) \subset c_2 (\mathcal{X})$.
\end{definition}
Our work does not focus on this type of cost functions, but a natural question is the Zig-Zag Strategy occur when the model requires that type of restricted cost function? Is there something special about the fact we use the Euclidean metric?
The answer is \emph{no} as  we show below. 
%shown in  Figure \ref{fig: seperable}.

In particular, consider the special case of linear cost functions, where cost a given $\alpha \in \mathbb{R}^d$, cost is given by 
\[  c(x,y) = \langle \alpha, (y-x) \rangle_{+} \]

Imagine a screening process with two classifiers in two dimensions with a small angle between them. In this special cost where the cost vector $\alpha$
is $[0,1]$, i.e. a vector straight upwards from the origin a Zig Zag Strategy exists. 

Observe that any point in the cone region between the two classifiers can evade the screening process by zigging right then left, with no upward movement. Since these shift vectors are orthogonal to $\alpha$, they require zero cost!

\begin{comment}
\begin{figure}[h!]
\label{fig: seperable}
\centering
\label{fig: naive}
\includegraphics[width=0.5\textwidth]{figures/seperablelb}
\caption{In this case $\alpha$ is the cost vector for a linear cost function. 
Observe that any point in the cone region can evade the screenign process by zigging right then left, with no upward movement. Since these shift vectors are orthogonal to $\alpha$, they require zero cost!}
\centering
\end{figure}
This Zig-Zag Strategy can hold generically when $\alpha$ angle less than $90$ degrees  with at least one of $h_1$ or $h_2$. 
\end{comment}


==> sup-6_hardness.tex <==


\begin{proof}
\label{hardnessproof}
\juba{not formal enough yet. We need to start by setting up the problem of Bruckner or Moritz' paper (single classifier $h$) formally, then formally state the corresponding instance to our problem $(h_0,\ldots,h_0,h)$. Let's be clear what is an instance of what problem too.}
    For a given instance of strategic classification, we can reduce finding a hypothesis $h$ that attains the strategic optimum for that problem to solving for the strategic screening process.

    Consider a pipeline $\mathcal{P}=\{h_0, \dots h_0, h \} $ where the first $k-1$ classifier is the all zero linear classifier (so any point $x \in \mathcal{X}$ passes these classifiers) and the last classifier is $h$.

    Since any point $x$ passes these $k-1$ stages, they do not need to manipulate and can reserve all of their manipulation cost for the last stage. 
    Thus the best response of an actor at $x$ for evading the screening process is identical to a best response for getting the positive classification for just $h$. Thus $h$ and $\mathcal{P}$ have the same optimal strategic accuracy and an optimal defense for the classifiers in $\mathcal{P}$ is the same as just for $h$. 
    
    Given an single classifier $w$, we can thus embed it into a pipeline such that the strategic optimum and any Agent's strategy is identical and thus solving for Strategic Screening is at least as hard as strategic classification, even for linear classifiers, using the hardness result in Section 3.1 of \cite{bruckner2011stackelberg}.
    %However, observe that the assumptions for our setting are more specific than that of \cite{hardt2016strategic}, in particular we want hardness for linear classifiers and the Eucliedan Metric. 
\end{proof}

%\begin{lemma}
%The construction in \cite{hardt2016strategic} can be done in three dimensions the euclidean metric. The key feature is we need to show we can implement the metric in theorem 4.1 
%\end{lemma}

%\begin{proof}
    
%\end{proof}

==> sup7fairness.tex <==
\paragraph{Fairness and Strategic Screening} %As noted in the related work section, there are multiple works that consider fairness and strategic manipulation. 
\ref{app:fairness}

Some of the works cited in the related work section consider fairness considerations in the space of strategic manipulation, stemming either from unequal abilities to manipulate~\cite{socialcost18,hu2019disparate} or unequal access to information about the classifiers~\cite{bechavod2022information} across different groups. We do not consider these connections in our work, but these considerations are of significant interest and a natural direction for further research, especially due to the importance of making fair decision in high-stake, life altering contexts. We finish with a few interesting examples for this.

Disparities might arise both in the conjunction and in the sequential setting, with or without defense. 
Consider the classifiers presented in Example \ref{exp:zigzag} and an instance in which candidates belong to two groups, $G^1$ and $G^2$ with initial feature vector distributed identically and characterized by different total manipulation budgets,  $\sqrt{2}=\tau^2>\tau^1=5/4$. 
The narrative of the fairness disparities in the conjunction case is a simple generalization of the single classifiers case (e.g., \cite{hardt2016strategic})- If the distribution is such that a significant fraction of individuals (from both groups) starts at a feature vector that is classified by both classifiers as $0$ and that requires $\sqrt{2}$ manipulation cost to reach their intersection--- only the individuals form $G_2$ will be able to manipulate. 
For the sequential case, consider a distribution with a large enough fraction of individuals starting  at $(0,0)$. Example \ref{exp:zigzag} demonstrates that only individuals from $G_2$ will have sufficient budget to manipulate (using the zig-zag strategy). 
If the firm will apply the conservative defense, individuals from $G_1$ that should have been classified as positive might not have sufficient  budget to manipulate their way to acceptance,  which in turn implies  higher false negative rates. 
This indicates, similarly to prior results in strategic classification (e.g.,~\cite{hu2019disparate}), how the  members of the advantaged group are more  easily admitted/hired. 
